Guided Trajectory Generation with Diffusion Models for Offline Model-based Optimization

Optimizing complex and high-dimensional black-box functions is ubiquitous in science and engineering fields. Unfortunately, the online evaluation of these functions is restricted due to time and safety constraints in most cases. In offline model-based optimization (MBO), we aim to find a design that maximizes the target function using only a pre-existing offline dataset. While prior methods consider forward or inverse approaches to address the problem, these approaches are limited by conservatism and the difficulty of learning highly multi-modal mappings. Recently, there has been an emerging paradigm of learning to improve solutions with synthetic trajectories constructed from the offline dataset. In this paper, we introduce a novel conditional generative modeling approach to produce trajectories toward high-scoring regions. First, we construct synthetic trajectories toward high-scoring regions using the dataset while injecting locality bias for consistent improvement directions. Then, we train a conditional diffusion model to generate trajectories conditioned on their scores. Lastly, we sample multiple trajectories from the trained model with guidance to explore high-scoring regions beyond the dataset and select high-fidelity designs among generated trajectories with the proxy function. Extensive experiment results demonstrate that our method outperforms competitive baselines on Design-Bench and its practical variants. The code is publicly available in \texttt{https://github.com/dbsxodud-11/GTG}.

==> tables/median.tex <==
\begin{table*}[h]
\caption{Experiments on Design-Bench Tasks. We report the median (50th percentile) among $Q$=128 candidates. \textbf{\textcolor{blue}{Blue}} denotes the best entry in the column, and
\textbf{\textcolor{violet}{Violet}} denotes the second best.}
\centering
% \vspace{-7pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Method}  & TFBind8 & TFBind10 & Superconductor & Ant & D'Kitty & Mean Rank\\
\midrule
$\mathcal{D}$ (best) & 0.439 & 0.467 & 0.399 & 0.565 & 0.884 & -\\
\midrule
% \multirow{4}{*}{Traditional} 
BO-qEI &  0.439 ± 0.000 &  0.467 ± 0.001 &  0.344 ± 0.024 &   0.569 ± 0.000 &  0.883 ± 0.000 & 11 / 15\\
CMA-ES &  0.543 ± 0.009 &  0.484 ± 0.017 &  0.376 ± 0.005 &  -0.041 ± 0.008 &  0.678 ± 0.015 & 8.4 / 15\\  
REINFORCE &  0.453 ± 0.015 &  0.470 ± 0.004 &  0.471 ± 0.017 &   0.137 ± 0.038 &  0.447 ± 0.179 & 11.6 / 15\\ 
Grad Ascent &  0.617 ± 0.027 &  0.466 ± 0.004 &  0.477 ± 0.024 &   0.148 ± 0.012 &  0.541 ± 0.195 & 7.6 / 15\\ 
\midrule
% \multirow{5}{*}{Surrogate-based}
COMs &  0.470 ± 0.019 &  0.473 ± 0.014 &  0.388 ± 0.026 &   0.529 ± 0.024 &  0.886 ± 0.001 & 8.2 / 15 \\
NEMO & 0.438 ± 0.001 & 0.454 ± 0.001 & 0.318 ± 0.008 & 0.592 ± 0.000 & 0.880 ± 0.000 & \textbf{\textcolor{violet}{4.8 / 15}}\\   
RoMA & 0.555 ± 0.020 & 0.512 ± 0.020 & 0.372 ± 0.019 &  0.479 ± 0.041 &  0.853 ± 0.007 & 6.6 / 15\\ 
BDI & 0.595 ± 0.000 & 0.467 ± 0.001 & 0.395 ± 0.019 & 0.556 ± 0.000 & 0.878 ± 0.000 & 6.4 / 15\\
ICT & 0.514 ± 0.015 & 0.447 ± 0.004 & 0.341 ± 0.013 & 0.526 ± 0.008 & 0.880 ± 0.002 & 7 / 15\\
\midrule
% \multirow{3}{*}{Generative-based}
CbAS &  0.424 ± 0.021 &  0.459 ± 0.004 &  0.127 ± 0.015 &  0.377 ± 0.036 &  0.747 ± 0.019 & 10.8 / 15\\
MINs &  0.426 ± 0.017 &  0.468 ± 0.007 &  0.341 ± 0.017 &   0.636 ± 0.020 &  0.890 ± 0.003 & 8.4 / 15\\
DDOM & 0.508 ± 0.011 & 0.450 ± 0.007 & 0.274 ± 0.010 & 0.125 ± 0.005 & 0.310 ± 0.000 & 9.6 / 15\\  
\midrule
% \multirow{3}{*}{Sequential Modeling}
BONET & 0.421 ± 0.065 & 0.469 ± 0.033 & 0.344 ± 0.021 & 0.802 ± 0.032 & 0.907 ± 0.009 & 10 / 15\\ 
PGS &  &  & 0.267 ± 0.058 & 0.199 ± 0.014 & 0.883 ± 0.003 & 7.4 / 15\\ 
\midrule
\textbf{GTG (Ours)} & 0.568 ± 0.062
 & 0.447 ± 0.019 & 0.264 ± 0.032 & 0.805 ± 0.025
 & 0.922 ± 0.005 & \textbf{\textcolor{blue}{1.6 / 15}}\\ 
\bottomrule
\end{tabular}}
\label{table:median}
\end{table*}
